Towards Painless Policy Optimization for Constrained MDPs

We study policy optimization in an infinite horizon, $\gamma$-discounted constrained Markov decision process (CMDP). Our objective is to return a policy that achieves large expected reward with a small constraint violation. We consider the online setting with linear function approximation and assume global access to the corresponding features. We propose a generic primal-dual framework that allows us to bound the reward sub-optimality and constraint violation for arbitrary algorithms in terms of their primal and dual regret on online linear optimization problems. We instantiate this framework to use coin-betting algorithms and propose the Coin Betting Politex (CBP) algorithm. Assuming that the action-value functions are $\varepsilon_b$-close to the span of the $d$-dimensional state-action features and no sampling errors, we prove that $T$ iterations of CBP result in an $O\left(\frac{1}{(1 - \gamma)^3 \sqrt{T}} + \frac{\varepsilon_b\sqrt{d}}{(1 - \gamma)^2} \right)$ reward sub-optimality and an $O\left(\frac{1}{(1 - \gamma)^2 \sqrt{T}} + \frac{\varepsilon_b \sqrt{d}}{1 - \gamma} \right)$ constraint violation. Importantly, unlike gradient descent-ascent and other recent methods, CBP does not require extensive hyperparameter tuning. Via experiments on synthetic and Cartpole environments, we demonstrate the effectiveness and robustness of CBP.

==> Algorithm.tex <==
\section{Algorithm}
\label{sec:Algorithm}

\begin{algorithm}[!h]
\caption{CMDP-Politex}
\label{alg:cmdp-politex}
\begin{algorithmic}[1]
    \State \textbf{Input}: $\pi_0$ (policy initialization), $\lambda_0 = 0$ (dual variable initialization), $T$ (Number of iterations), $\eta_1$ (Step-size for primal update), $\eta_2$ (Step-size for dual update), Feature map $\Phi: \mathcal{S} \times \mathcal{A} \rightarrow d$. 
    
    \State Given $\Phi$, find $\cZ \subset \mathcal{S} \times \mathcal{A}$ and $\mu$ as in the Kiefer-Wolfowitz theorem. 
    
    \For{$t = 0$, \dots,  $T-1$}
    
    \State Roll out with policy $\pit$ for $H$ steps to get targets for $\hat{r}(z)$ and $\hat{c}(z)$ for $z \in \cZ$. 
    
    \State Solve weighted least squares: 
    \begin{align}
    \hat{\theta}_{r} = \argmin_{\theta \in \R^d} \sum_{z \in \cZ} \mu(z) \left(\langle \theta, \phi(z) \rangle - \hat{r}(z) \right)^2 \\
    \hat{\theta}_{c} = \argmin_{\theta \in \R^d} \sum_{z \in \cZ} \mu(z) \left(\langle \theta, \phi(z) \rangle - \hat{c}(z) \right)^2
    \end{align}
    
    \State Update estimates $\forall (s,a) \in \cZ$:
    \begin{align}
    \rewardqhat{t}(s,a) & = \langle \hat{\theta}_{r}, \phi(s,a) \rangle \, ; \quad \constqhat{t}(s,a) = \langle \hat{\theta}_{c}, \phi(s,a) \rangle \nonumber \\
    \lagqhat{t}(s,a) & = \rewardqhat{t}(s,a) + \lambda_{t} \, \constqhat{t}(s,a)  \\
    \consthat{t}(s) & = \pit(a | s) \constqhat{t}(s,a) 
    \end{align}
    
    \State Update the primal variables (policy) using OMD, and use OGD for the dual variables (Lagrange multipliers), 
    \begin{align}
    \pitt(a|s) & = \frac{\pit(a|s) \exp\left(\eta_1 \lagqhat{t}(s,a) \right)
    }{\sum_{a'}\pit(a'|s)\exp\left(\eta_1 \lagqhat{t}(s,a') \right)} \label{eq:primal-update} \tag{Primal update} \\
    \lambdatt & = \cP_{[0, 2 U]}[\lambdat - \eta_2 \, (\consthat{t} - b)].\label{eq:dual-update} \tag{Dual update}
    \end{align}
    
    \EndFor
    
    \State Return $\pi_{T}$. 
\end{algorithmic}
\end{algorithm}
    
%%%%%%%%%%%%%%%%%%%%%%
Coin Betting Politex
\section{Algorithm}
\label{sec:Algorithm}

\begin{algorithm}[!h]
\caption{CBP}
\label{alg:cmdp-politex}
\begin{algorithmic}[1]
    \State \textbf{Input}: $\pi_0$ (policy initialization), $\lambda_0$ (dual variable initialization), $T$ (Number of iterations), $\alpha_\lambda2$ (Step-size for dual update), Feature map $\Phi: \mathcal{S} \times \mathcal{A} \rightarrow d$. 
    
    \State Given $\Phi$, find $\cZ \subset \mathcal{S} \times \mathcal{A}$ and $\mu$ as in the Kiefer-Wolfowitz theorem. 
    
    \For{$t = 0$, \dots,  $T-1$}
    
    \State Roll out with policy $\pit$ for $H$ steps to get targets for $\hat{r}(z)$ and $\hat{c}(z)$ for $z \in \cZ$. 
    
    \State Solve weighted least squares: 
    \begin{align}
    \hat{\theta}_{r} = \argmin_{\theta \in \R^d} \sum_{z \in \cZ} \mu(z) \left(\langle \theta, \phi(z) \rangle - \hat{r}(z) \right)^2 \\
    \hat{\theta}_{c} = \argmin_{\theta \in \R^d} \sum_{z \in \cZ} \mu(z) \left(\langle \theta, \phi(z) \rangle - \hat{c}(z) \right)^2
    \end{align}
    
    \State Update estimates $\forall (s,a) \in \cZ$:
    \begin{align}
    \rewardqhat{t}(s,a) & = \langle \hat{\theta}_{r}, \phi(s,a) \rangle \, ; \quad \constqhat{t}(s,a) = \langle \hat{\theta}_{c}, \phi(s,a) \rangle \nonumber \\
    \lagqhat{t}(s,a) & = \rewardqhat{t}(s,a) + \lambda_{t} \, \constqhat{t}(s,a)  \\
    \consthat{t}(s) & = \pit(a | s) \constqhat{t}(s,a) 
    \end{align}
    
    \State Update the primal variables (policy) using OMD, and use OGD for the dual variables (Lagrange multipliers), 
    \begin{align}
    \pitt(a|s) & = \frac{\pit(a|s) \exp\left(\eta_1 \lagqhat{t}(s,a) \right)
    }{\sum_{a'}\pit(a'|s)\exp\left(\eta_1 \lagqhat{t}(s,a') \right)} \label{eq:primal-update} \tag{Primal update} \\
    \lambdatt & = \cP_{[0, 2 U]}[\lambdat - \eta_2 \, (\consthat{t} - b)].\label{eq:dual-update} \tag{Dual update}
    \end{align}
    
    \EndFor
    
    \State Return $\pi_{T}$. 
\end{algorithmic}
\end{algorithm}

==> App-algorithm.tex <==
\section{Additional Algorithms}
\label{app:algorithms}


